$FastDoc$: Domain-Specific Fast Continual Pre-training Technique using Document-Level Metadata and Taxonomy

In this paper, we propose $FastDoc$ (Fast Continual Pre-training Technique using Document Level Metadata and Taxonomy), a novel, compute-efficient framework that utilizes Document metadata and Domain-Specific Taxonomy as supervision signals to continually pre-train transformer encoder on a domain-specific corpus. The main innovation is that during domain-specific pretraining, an open-domain encoder is continually pre-trained using sentence-level embeddings as inputs (to accommodate long documents), however, fine-tuning is done with token-level embeddings as inputs to this encoder. We perform such domain-specific pre-training on three different domains namely customer support, scientific, and legal domains, and compare performance on 6 different downstream tasks and 9 different datasets. The novel use of document-level supervision along with sentence-level embedding input for pre-training reduces pre-training compute by around $1,000$, $4,500$, and $500$ times compared to MLM and/or NSP in Customer Support, Scientific, and Legal Domains, respectively. The reduced training time does not lead to a deterioration in performance. In fact we show that $FastDoc$ either outperforms or performs on par with several competitive transformer-based baselines in terms of character-level F1 scores and other automated metrics in the Customer Support, Scientific, and Legal Domains. Moreover, reduced training aids in mitigating the risk of catastrophic forgetting. Thus, unlike baselines, $FastDoc$ shows a negligible drop in performance on open domain.

==> sections/analysis.tex <==
\section{\fpdm: How document-level supervision with sentence inputs helps in QA with token inputs}
\label{fpdm_analysis}
%corpus and learned E-Manual representations}

%We deep dive and try to find some of the reasons behind the superior performance in the task of Question Answer whose performance depends on the efficiency in which  similarity between are learned, perform an analysis of the E-Manuals in pre-training corpus, and the learned E-Manual representations during pre-training to show that pre-training using document level supervision indirectly provides supervision on local paragraph level context, and the representations learnt are independent to the type of input embeddings being used. 
Here, we deep dive further to analyze the following phenomena: (1). The pre-training phase brings embeddings of  similar documents together. However, the downstream tasks mainly depend on better estimation of similarity between sentences. We try to see why such \tb{transitivity} holds. We posit one of the reasons being very high similarity between `similar' documents. (2). Our encoder is pre-trained using sentence embedding inputs but is fine-tuned with token embedding inputs. We analyze if the relative document representations are independent to the type of input embeddings being used (A similar analysis of attention matrices is presented \textbf{\textit{in suppl.}}). 
%We then show that thus document level similarity are observed largely to the similar extent whether we consider sentence embedding or token embedding. 

%\pg{I feel that even if this needs to come in the main paper, this can come later in the analysis. If in appendix, we can just put a line here.}
% \noindent
\noindent\textbf{Learning Local Context with Document-level Supervision:} 
We contrast the paragraph-level similarity between similar and dissimilar E-Manuals used during pre-training. Given a pair of E-Manuals, each paragraph in the two E-Manuals is converted to a fixed-size vector using Doc2Vec model \citep{doc2vec} trained on Wikipedia, and the similarity score (cosine) with the most similar paragraph from the other E-Manual is considered as a `Paragraph Similarity Score'. The distribution of this score across similar and dissimilar document pairs is plotted in Fig.~\ref{fig:para_sim_1}.

\begin{figure}[!thb]
    \centering
    \includegraphics[width=0.35\textwidth]{images/only_para_similarity.png}
    \caption{Distribution of `Paragraph Similarity Score' across similar and dissimilar document pairs}
    \label{fig:para_sim_1}
\end{figure}

We can infer that paragraph pairs from similar documents are skewed towards higher similarity, with more than half of the samples having a `Paragraph Similarity Score' > $0.7$. The sections where the similarity is even higher are mainly the specific sections where some procedure/task is specified like `How to calibrate a wireless thermometer?' or the device specifications and/or warnings about using the device/service are given, which would indirectly help the model in the downstream QA task. Similarly, (even the most similar) paragraph pairs in dissimilar documents are skewed towards lower similarity, with a  majority of the samples having a `Paragraph Similarity Score' < $0.5$. Thus similar documents have very-similar local (paragraph-level) contexts, suggesting that, using document-level supervision during pre-training also helps in learning local contexts.  %To test this more explicitly we perform the next experiment. 
%This would help in improving performance on downstream sentence and paragraph level tasks.

\noindent\textbf{Qualitative Evaluation of  Relative Document Representations: }

%\pg{I have similar comments as on earlier experiment. Not sure if it is really helping. Can be removed / moved.}
%\abhi{moved attention matrices to suppl.}

We analyze the relative document representations learnt by the pre-trained encoder in $\fpdm_{RoBERTa}$, for both sentence-level and token-level input embeddings. 
%In this experiment, we show that the relative representations of E-Manuals is independent of whether we take sentence or token embeddings as inputs to the transformer encoder pre-trained using document level supervision. %, and thus, it gives good results when token embeddings are inputs during fine-tuning. 
For $4$ different product categories (printer, plumbing product, battery charger, indoor furnishings), we consider $5$ E-Manuals each containing between $400-512$ tokens %(using both BERT as well as RoBERTa subword tokenizers, including special tokens) 
 so that it complies with the %. The number of tokens considered is less than $512$, as that is the 
maximum number of tokens accepted by \bert or \rbe as inputs. %When token-level embeddings are inputs, the output corresponding to the special classification token \cite{bert, roberta} is the document representation. When sentence-level embeddings are inputs, the document representation is found in the same way as during pre-training.
The cosine similarity between the E-Manual representations of each of the $190$ E-Manual pairs corresponding to both types of input embeddings is obtained, and normalized (using max-min normalization). The similarity values are positively correlated to each other, with the Pearson Correlation value being $0.515$. %If we calculate the correlation among datapoints within each category, and then average over all categories, we get a similar correlation of $0.512$. Also, 
We, further, take the category-wise average representations, and repeat this experiment. We find that the Pearson Correlation for the similarity values is $0.977$. Hence, the relative representations in both the representation spaces are highly correlated, which justifies the reason for good downstream performance when an encoder pre-trained on sentence embedding inputs is fine-tuned on token embedding inputs. A visual comparison of the learnt representations is described \textbf{\emph{in suppl.}}
